A General Framework For Constructing Locally Self-Normalized Multiple-Change-Point Tests

We propose a general framework to construct self-normalized multiple-change-point tests with time series data. The only building block is a user-specified one-change-point detecting statistic, which covers a wide class of popular methods, including cumulative sum process, outlier-robust rank statistics and order statistics. Neither robust and consistent estimation of nuisance parameters, selection of bandwidth parameters, nor pre-specification of the number of change points is required. The finite-sample performance shows that our proposal is size-accurate, robust against misspecification of the alternative hypothesis, and more powerful than existing methods. Case studies of NASDAQ option volume and Shanghai-Hong Kong Stock Connect turnover are provided.

==> myFrontMatters.tex <==
%----------------------------------------
% Paper Title
%----------------------------------------
\if1\blind
{
  \title{\bf A General Framework For Constructing Locally Self-Normalized Multiple-Change-Point Tests}
  \author{Kin Wai Chan
				\thanks{Department of Statistics, The Chinese University of Hong Kong.
				Email: {kinwaichan@cuhk.edu.hk}} \\
				The Chinese University of Hong Kong
			\and
			Cheuk Hin Cheng 
				\thanks{Department of Statistics, The Chinese University of Hong Kong.
				Email: {andychengcheukhin@link.cuhk.edu.hk}} \\
				The Chinese University of Hong Kong
		}
  \maketitle
} \fi

\if0\blind
{
  \bigskip
  \bigskip
  \bigskip
  \begin{center}
    {\LARGE\bf Multiple Change Point Test With Application of Self Normalization and Localized CUSUM}
\end{center}
  \medskip
} \fi	
\maketitle


==> myPreliminary.tex <==
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Packages 
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
\usepackage{varioref} 
\usepackage{xr-hyper} 
\usepackage[colorlinks]{hyperref}
\usepackage{booktabs}
\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}
\usepackage{epsfig,amsmath,amssymb,euscript,amsfonts,hyperref}
\usepackage{natbib}	
\usepackage{array}
\usepackage{nccbbb}
\usepackage{verbatim} 
\usepackage[lined,boxed,commentsnumbered, ruled,linesnumbered, algosection]{algorithm2e} 
\usepackage{graphicx}
\usepackage{bm}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{bbold}
\usepackage[cal=boondox]{mathalfa} 
\usepackage{comment}
\usepackage{enumerate}
\usepackage{color}
\usepackage{caption,setspace}						
\captionsetup{font={small,stretch=1},labelfont=bf} 
\usepackage{lipsum}
\usepackage{float}
\usepackage{xcolor}
\usepackage{makecell}
\setcellgapes{2pt}
\usepackage{authblk}
\usepackage{marginnote}
\usepackage[normalem]{ulem} 
\usepackage{cancel} 
\usepackage{textcomp} 
\usepackage{enumitem} 


%% Tables fixed width
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Margins
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\topfraction}{0.95}
\renewcommand{\textfraction}{0.05}

\addtolength{\oddsidemargin}{-.5in}%
\addtolength{\evensidemargin}{-.5in}%
\addtolength{\textwidth}{1in}%
\addtolength{\textheight}{1.3in}%
\addtolength{\topmargin}{-.8in}%


\def\spacingset#1{\renewcommand{\baselinestretch}%
{#1}\small\normalsize} \spacingset{1}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Theorem Style
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\numberwithin{equation}{section}  
\numberwithin{table}{section} 
\numberwithin{figure}{section}  
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{principle}{Principle}[section]

\theoremstyle{definition}
\newtheorem{example}{Example}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{model}{Model}[section]

\hypersetup{citecolor=myblue, linkcolor=myred, urlcolor=myblue}




%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### color
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\definecolor{BUred}{rgb}{0.8, 0.0, 0.0}
\definecolor{BLUE}{rgb}{0.0, 0.28, 0.67}
\definecolor{magenta}{rgb}{1,0,.6}
\definecolor{blue0}{rgb}{0.95, 0.97, 1.0}
\definecolor{brown}{rgb}{0.75, 0.25, 0.0}

\usepackage{color}
	\definecolor{brown}{rgb}{0.75, 0.25, 0.0}
	\definecolor{mygreen}{rgb}{0.1, 0.5, 0.1}	
	\definecolor{myred}{rgb}{0.7, 0.1, 0.1}
	\definecolor{myblue}{rgb}{0.1, 0.1, 0.7}
	\definecolor{mygold}{rgb}{0.95, 0.85, 0.37}
	\definecolor{mygray}{rgb}{0.5,0.5,0.5}
	\definecolor{myorange}{rgb}{1,0.5,0}



%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### marginnote
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\newcommand{\note}[1]{\reversemarginpar\marginnote{\scriptsize \color{myred}\!\!\!\!\!\!\!\!\!\!\!\!\!\begin{minipage}{0.15\textwidth}[\textsf{KW:  #1}]\end{minipage}}}
\newcommand{\notealso}[1]{\normalmarginpar\marginnote{\scriptsize \color{myred}\!\!\!\!\!\begin{minipage}{0.15\textwidth}[\textsf{KW:  #1}]\end{minipage}}}



\newcommand{\add}[2][]
{\ifnum\revise=0{#1}\fi
\ifnum\revise=1{\color{myred}#2}\fi
\ifnum\revise=2{\color{black}#2}\fi
\ifnum\revise=3{{\color{mygray}\sout{#1}}{\color{myred}#2}}\fi
}
\newcommand{\del}[1]
{\ifnum\revise=0{#1}\fi
\ifnum\revise=1{\color{myred}\sout{#1}}\fi
\ifnum\revise=2\fi
\ifnum\revise=3{\color{myred}\sout{#1}}\fi
}




%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Operators 
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	

% mathematics 
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\vech}{\mathop{\mathrm{vech}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mean}{mean}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\expit}{expit}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\comp}{\textsc{comp}}
\newcommand{\T}{\textsc{T}}
\newcommand{\D}{\textnormal{d}}
\newcommand{\dd}{\,\textnormal{d}}


% probability 
\newcommand{\pr}{\mathsf{P}} 
\newcommand{\E}{\mathsf{E}} 
\newcommand{\median}{\mathop{\mathsf{median}}}
\newcommand{\Cov}{\mathop{\mathsf{Cov}}} 
\newcommand{\Var}{\mathop{\mathsf{Var}}}
\newcommand{\var}{\mathop{\mathsf{var}}}
\newcommand{\Bias}{\mathop{\mathsf{Bias}}}
\newcommand{\bias}{\mathop{\mathsf{bias}}}
\newcommand{\AMSE}{\mathop{\mathsf{AMSE}}}
\newcommand{\SMSE}{\mathop{\mathsf{SMSE}}}
\newcommand{\MSE}{\mathop{\mathsf{MSE}}}
\newcommand{\CSD}{\mathop{\mathsf{CSD}}} 


% convergence and distribution relation 
\newcommand{\inD}{   \overset{ \textnormal{d}   }{\rightarrow} }
\newcommand{\inWPone}{   \overset{ \textnormal{wp1}   }{\rightarrow} }
\newcommand{\inAS}{   \overset{ \textnormal{a.s.}   }{\rightarrow} }
\newcommand{\inP}{  \overset{ \textnormal{pr}    }{\rightarrow} }
\newcommand{\inLp}{ \overset{ \mathcal{L}^p }{\rightarrow} }
%\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern4mu{#1#2}}}
\newcommand{\eqD}{   \overset{ \text{$\mathcal{D}$}   }{=} }
\newcommand{\iid}{\textsc{iid}} 
\newcommand{\simIID}{   \overset{ \iid   }{\sim} }
\newcommand{\simIND}{   \overset{ {\indep}   }{\sim} }
\newcommand{\simApprox}{   \dot{\sim} }


% statistics 
\newcommand{\RV}{\textsc{rv}}
\newcommand{\cdf}{\textsc{cdf}} 
\newcommand{\cgf}{\textsc{cgf}} 
\newcommand{\pdf}{\textsc{pdf}} 
\newcommand{\pmf}{\textsc{pmf}} 
\newcommand{\chf}{\textsc{chf}} 
\newcommand{\mgf}{\textsc{mgf}}
\newcommand{\EF}{\textsc{EF}}
\newcommand{\NEF}{\textsc{NEF}}
\newcommand{\MLE}{\textsc{MLE}}
\newcommand{\JS}{\textsc{JS}}
\newcommand{\MAP}{\textsc{MAP}}
\newcommand{\Med}{\textsc{Med}}
\newcommand{\MME}{\textsc{MME}}
\newcommand{\GMME}{\textsc{GMME}}
\newcommand{\minimax}{\textsc{M}}
\newcommand{\Bayes}{\textsc{Bayes}}
\newcommand{\Adm}{\textsc{A}}
\newcommand{\HPD}{\textsc{HPD}}
\newcommand{\ET}{\textsc{ET}}

% distribution 
\newcommand{\Bern}{\textnormal{Bern}} 
\newcommand{\Unif}{\textnormal{Unif}} 
\newcommand{\Logistic}{\textnormal{Logistic}} 
\newcommand{\Normal}{\textnormal{N}} 
\newcommand{\logNormal}{\textnormal{LN}} 
\newcommand{\Bin}{\textnormal{Bin}} 
\newcommand{\NB}{\textnormal{NB}} 
\newcommand{\HG}{\textnormal{HG}} 
\newcommand{\Geom}{\textnormal{Geom}} 
\newcommand{\Beta }{\textnormal{Beta}} 
\newcommand{\BetaBin}{\textnormal{Beta-Bin}}
\newcommand{\Ga}{\textnormal{Ga}} 
\newcommand{\Exp}{\textnormal{Exp}} 
\newcommand{\Expo}{\textnormal{Expo}} 
\newcommand{\Po}{\textnormal{Po}} 
\newcommand{\Multi}{\textnormal{Multi}} 
\newcommand{\Wishart}{\textnormal{Wishart}} 
\newcommand{\MIG}{\textnormal{MIG}} 
\newcommand{\student}{\textnormal{t}} 
\newcommand{\Cauchy}{\textnormal{Cauchy}} 
\newcommand{\Pareto}{\textnormal{Pareto}} 
\newcommand{\Laplace}{\textnormal{Laplace}} 
\newcommand{\Dir}{\textnormal{Dir}} 
\newcommand{\DP}{\textnormal{DP}} 
\newcommand{\Inv}{\textnormal{Inv-}} 
\newcommand{\F}{\textnormal{F}} 
\newcommand{\Supp}{\textnormal{Supp}} 
\newcommand{\round}{\textnormal{round}} 


% for recursive TAVC estimation 
\newcommand{\NBM}{\mathop{\mathrm{NBM}}}
\newcommand{\OBM}{\mathop{\mathrm{OBM}}}
\newcommand{\HOC}{\mathop{\mathrm{HOC}}}
\newcommand{\QS}{\mathop{\mathrm{QS}}}
\newcommand{\PSR}{ \textnormal{\tiny{P}} }
\newcommand{\TSR}{ \textnormal{\tiny{T}} }
\newcommand{\TRI}{ \triangle }


% Andy's notations (10 May 2021)
\newcommand{\BM}{ \mathbb{B}}
\def\shao{\textsc{S}}
\def\KS{\textsc{KS}}
\def\zhang{\textsc{Z}}
\def\T{\textsc{T}}
\def\L{\textsc{L}}
\def\V{\textsc{V}}
\def\C{\textsc{C}}
\def\D{\textsc{D}}
\def\Y{\textsc{Y}}
\def\W{\textsc{W}}
\def\H{\textsc{H}}
\def\G{\textsc{G}}
\def\Q{\textsc{Q}}
\def\IF{\textsc{IF}}
\def\KS{\textsc{KS}}
\def\I{\textsc{I}}






